RobustSeiz: a model-agnostic framework for auditing the recording-environment, noise and adversarial robustness of EEG seizure detectors

Background and Objective: Automated electroencephalography (EEG) seizure detectors are validated on clean research recordings, whereas clinical recordings are altered by electrode problems, equipment settings and artifacts. As seizure treatment is time-critical, we tested whether detectors stay reliable and timely under such conditions. Methods: We developed RobustSeiz, an open-source framework that audits any trained detector without modifying it. Its novelty is the evaluation pipeline, not a new detector: a model-agnostic protocol applying controlled, seeded shifts (recording environment, noise and artifacts, worst-case adversarial), scoring that adds onset timing and model uncertainty to event-based accuracy, and paired statistics against clean recordings. We audited four deep-learning detectors on three public datasets unseen in training. Results: Robustness varied widely and was independent of clean accuracy. Adversarial changes of 5-10% of signal amplitude reduced the F1-score by up to 0.57, and electrode-contact noise silently lowered sensitivity from 0.57 to 0.06. Shifts delayed the seizures still detected by up to 62 s. Read with accuracy, dropout certainty fell under filtering shifts but rose as noise silenced detection; only a quarter of failures lowered it. Conclusions: Clean accuracy alone does not establish reliability or timeliness. RobustSeiz makes pre-deployment robustness audits reproducible.

==> tables/tab_baselines.tex <==
SeizureTransformer & TUSZ & 43 & 195/340 & \makecell{0.57\\{\scriptsize [0.40, 0.72]}} & \makecell{0.69\\{\scriptsize [0.53, 0.78]}} & \makecell{0.62\\{\scriptsize [0.46, 0.73]}} & \makecell{16.7\\{\scriptsize [10.2, 24.4]}} & 0.46 \\
EEGNet & TUSZ & 43 & 196/340 & \makecell{0.58\\{\scriptsize [0.41, 0.71]}} & \makecell{0.57\\{\scriptsize [0.42, 0.70]}} & \makecell{0.57\\{\scriptsize [0.44, 0.66]}} & \makecell{28.0\\{\scriptsize [13.2, 45.4]}} & 0.36 \\
EEGWaveNet & TUSZ & 43 & 161/340 & \makecell{0.47\\{\scriptsize [0.35, 0.59]}} & \makecell{0.29\\{\scriptsize [0.17, 0.43]}} & \makecell{0.36\\{\scriptsize [0.24, 0.48]}} & \makecell{74.3\\{\scriptsize [57.2, 93.4]}} & 0.10 \\
EventNet & TUSZ & 43 & 219/340 & \makecell{0.64\\{\scriptsize [0.48, 0.77]}} & \makecell{0.78\\{\scriptsize [0.63, 0.88]}} & \makecell{0.71\\{\scriptsize [0.56, 0.81]}} & \makecell{11.3\\{\scriptsize [5.7, 19.4]}} & 0.54 \\
\addlinespace
EEGNet & Siena & 14 & 31/47 & \makecell{0.66\\{\scriptsize [0.47, 0.82]}} & \makecell{0.42\\{\scriptsize [0.28, 0.64]}} & \makecell{0.51\\{\scriptsize [0.37, 0.69]}} & \makecell{7.3\\{\scriptsize [3.4, 11.0]}} & 0.30 \\
EEGWaveNet & Siena & 14 & 36/47 & \makecell{0.77\\{\scriptsize [0.58, 0.95]}} & \makecell{0.04\\{\scriptsize [0.03, 0.07]}} & \makecell{0.08\\{\scriptsize [0.05, 0.13]}} & \makecell{139.6\\{\scriptsize [100.6, 179.9]}} & 0.02 \\
EventNet & Siena & 14 & 26/47 & \makecell{0.55\\{\scriptsize [0.33, 0.81]}} & \makecell{0.39\\{\scriptsize [0.20, 0.68]}} & \makecell{0.46\\{\scriptsize [0.26, 0.68]}} & \makecell{7.0\\{\scriptsize [2.8, 14.2]}} & 0.41 \\
\addlinespace
EEGNet & CHB-MIT & 23 & 151/200 & \makecell{0.76\\{\scriptsize [0.61, 0.87]}} & \makecell{0.05\\{\scriptsize [0.03, 0.09]}} & \makecell{0.09\\{\scriptsize [0.05, 0.16]}} & \makecell{73.8\\{\scriptsize [42.9, 110.7]}} & 0.10 \\


==> tables/tab_mcd.tex <==
Clean (absolute F1, $c$) & 0.62 & 0.975 & 0.57 & 0.996 & 0.36 & -- & 0.71 & -- & 0.51 & 0.998 & 0.08 & -- & 0.46 & -- & 0.09 & 0.952 \\
\midrule
\addlinespace[2pt]
Band-pass 0.5--25 Hz & \textbf{$-$0.07} & \rd{rdH}{$-$10\,\textsuperscript{H}} & $-$0.01 & \rd{rdW}{$-$3\,\textsuperscript{W}} & +0.03 & -- & 0.00 & -- & \textbf{$-$0.14} & \rd{rdH}{$-$3\,\textsuperscript{H}} & +0.05 & -- & +0.14 & -- & $-$0.02 & \rd{rdW}{$-$18\,\textsuperscript{W}} \\
Band-pass 0.5--40 Hz & \textbf{$-$0.07} & \rd{rdH}{$-$7\,\textsuperscript{H}} & +0.01 & \rd{rdW}{$-$1\,\textsuperscript{W}} & +0.04 & -- & $-$0.01 & -- & \textbf{$-$0.08} & \rd{rdH}{$-$0.7\,\textsuperscript{H}} & +0.04 & -- & +0.15 & -- & $-$0.01 & \rd{rdW}{$-$6\,\textsuperscript{W}} \\
Band-pass 1--40 Hz & \textbf{$-$0.18} & \rd{rdH}{$-$41\,\textsuperscript{H}} & \textbf{$-$0.08} & \rd{rdH}{$-$17\,\textsuperscript{H}} & +0.06 & -- & $-$0.02 & -- & \textbf{$-$0.26} & \rd{rdH}{$-$11\,\textsuperscript{H}} & +0.05 & -- & +0.13 & -- & \textbf{$-$0.03} & \rd{rdH}{$-$43\,\textsuperscript{H}} \\
\addlinespace[2pt]
Electrode loss O1, O2 & $-$0.02 & +9 & \textbf{$-$0.13} & \rd{rdO}{+3\,\textsuperscript{O}} & $-$0.04 & -- & \textbf{$-$0.03} & -- & \textbf{$-$0.29} & \rd{rdO}{+1\,\textsuperscript{O}} & +0.01 & -- & 0.00 & -- & \textbf{$-$0.03} & \rd{rdH}{$-$25\,\textsuperscript{H}} \\
Electrode loss T7, T8 & $-$0.03 & +13 & $-$0.06 & +2 & \textbf{$-$0.05} & -- & \textbf{$-$0.08} & -- & \textbf{$-$0.18} & \rd{rdU}{+0.3\,\textsuperscript{U}} & 0.00 & -- & $-$0.02 & -- & +0.01 & +15 \\
\addlinespace[2pt]
Sampling round-trip 200 Hz & 0.00 & +5 & 0.00 & $-$0.2 & 0.00 & -- & 0.00 & -- & 0.00 & 0 & 0.00 & -- & +0.01 & -- & 0.00 & +0.3 \\
Sampling round-trip 100 Hz & 0.00 & +3 & 0.00 & $-$0.3 & 0.00 & -- & +0.01 & -- & 0.00 & +0.1 & 0.00 & -- & +0.02 & -- & 0.00 & +0.1 \\
Sampling round-trip 50 Hz & $-$0.02 & $-$0.5 & $-$0.02 & \rd{rdW}{$-$3\,\textsuperscript{W}} & 0.00 & -- & 0.00 & -- & \textbf{$-$0.16} & \rd{rdH}{$-$5\,\textsuperscript{H}} & 0.00 & -- & +0.04 & -- & \textbf{$-$0.03} & \rd{rdH}{$-$25\,\textsuperscript{H}} \\
\addlinespace[2pt]
ADC 12 bit & 0.00 & +7 & 0.00 & 0 & 0.00 & -- & 0.00 & -- & 0.00 & 0 & 0.00 & -- & 0.00 & -- & 0.00 & +0.1 \\
ADC 10 bit, $\pm$100 \textmu V & +0.02 & $-$2 & +0.02 & 0 & 0.00 & -- & $-$0.02 & -- & \textbf{$-$0.13} & \rd{rdH}{$-$3\,\textsuperscript{H}} & +0.01 & -- & +0.09 & -- & $-$0.02 & \rd{rdW}{$-$24\,\textsuperscript{W}} \\
ADC 5 bit & $-$0.01 & +4 & $-$0.06 & +1 & $-$0.02 & -- & \textbf{$-$0.04} & -- & \textbf{$-$0.34} & \rd{rdH}{$-$3\,\textsuperscript{H}} & 0.00 & -- & \textbf{$-$0.20} & -- & $-$0.02 & \rd{rdW}{$-$14\,\textsuperscript{W}} \\
\addlinespace[2pt]
Impedance 0--1 Hz, 50 \textmu V & $-$0.07 & +24 & \textbf{$-$0.11} & \rd{rdO}{+3\,\textsuperscript{O}} & $-$0.02 & -- & $-$0.03 & -- & \textbf{$-$0.17} & \rd{rdO}{+1\,\textsuperscript{O}} & 0.00 & -- & $-$0.01 & -- & 0.00 & +5 \\
Impedance 0--1 Hz, 100 \textmu V & \textbf{$-$0.30} & \rd{rdO}{+24\,\textsuperscript{O}} & \textbf{$-$0.43} & \rd{rdO}{+3\,\textsuperscript{O}} & \textbf{$-$0.05} & -- & \textbf{$-$0.09} & -- & \textbf{$-$0.31} & \rd{rdO}{+2\,\textsuperscript{O}} & $-$0.01 & -- & $-$0.03 & -- & +0.02 & +14 \\
Impedance 0--1 Hz, 200 \textmu V & \textbf{$-$0.52} & \rd{rdO}{+24\,\textsuperscript{O}} & \textbf{$-$0.52} & \rd{rdO}{+3\,\textsuperscript{O}} & \textbf{$-$0.07} & -- & \textbf{$-$0.33} & -- & \textbf{$-$0.37} & \rd{rdO}{+2\,\textsuperscript{O}} & $-$0.02 & -- & $-$0.06 & -- & +0.02 & +28 \\
\addlinespace[2pt]
Drift, piecewise linear & 0.00 & +6 & 0.00 & $-$0.1 & 0.00 & -- & $-$0.01 & -- & 0.00 & +0.1 & $-$0.01 & -- & $-$0.04 & -- & 0.00 & 0 \\
Drift, random walk & 0.00 & +7 & 0.00 & \rd{rdW}{$-$0.2\,\textsuperscript{W}} & $-$0.02 & -- & $-$0.01 & -- & 0.00 & +0.1 & $-$0.01 & -- & $-$0.02 & -- & 0.00 & +0.3 \\
Drift, 0.2 Hz sine, 50 \textmu V & +0.05 & +21 & 0.00 & +0.3 & \textbf{$-$0.10} & -- & 0.00 & -- & 0.00 & 0 & $-$0.01 & -- & +0.02 & -- & 0.00 & +0.2 \\
\addlinespace[2pt]
AWGN 50 dB SNR & 0.00 & +5 & 0.00 & +0.1 & 0.00 & -- & 0.00 & -- & 0.00 & $-$0.1 & 0.00 & -- & 0.00 & -- & 0.00 & +0.2 \\
AWGN 20 dB SNR & 0.00 & +1 & $-$0.02 & +0.9 & 0.00 & -- & $-$0.01 & -- & $-$0.03 & +0.5 & 0.00 & -- & $-$0.01 & -- & 0.00 & +1 \\
AWGN 5 dB SNR & $-$0.05 & +12 & \textbf{$-$0.32} & \rd{rdO}{+3\,\textsuperscript{O}} & $-$0.02 & -- & \textbf{$-$0.07} & -- & \textbf{$-$0.33} & \rd{rdO}{+2\,\textsuperscript{O}} & $-$0.01 & -- & \textbf{$-$0.38} & -- & +0.01 & +8 \\
AWGN 2 dB SNR & $-$0.08 & +18 & \textbf{$-$0.43} & \rd{rdO}{+4\,\textsuperscript{O}} & $-$0.02 & -- & \textbf{$-$0.12} & -- & \textbf{$-$0.35} & \rd{rdO}{+2\,\textsuperscript{O}} & $-$0.01 & -- & \textbf{$-$0.38} & -- & +0.02 & +7 \\
AWGN 0 dB SNR & \textbf{$-$0.11} & \rd{rdO}{+18\,\textsuperscript{O}} & \textbf{$-$0.47} & \rd{rdO}{+4\,\textsuperscript{O}} & $-$0.02 & -- & \textbf{$-$0.14} & -- & \textbf{$-$0.34} & \rd{rdO}{+2\,\textsuperscript{O}} & \textbf{$-$0.02} & -- & \textbf{$-$0.39} & -- & +0.03 & +8 \\
\addlinespace[2pt]
Mains 60 Hz, 0.1$\times$ RMS & 0.00 & +4 & 0.00 & 0 & 0.00 & -- & $-$0.01 & -- & 0.00 & +0.2 & 0.00 & -- & 0.00 & -- & 0.00 & 0 \\
Mains 60 Hz, 0.5$\times$ RMS & +0.01 & +7 & 0.00 & +0.9 & $-$0.02 & -- & \textbf{$-$0.04} & -- & $-$0.02 & +0.5 & $-$0.01 & -- & $-$0.03 & -- & 0.00 & +0.7 \\
Mains 60 Hz, 1$\times$ RMS & +0.03 & +10 & $-$0.01 & +2 & \textbf{$-$0.06} & -- & \textbf{$-$0.09} & -- & \textbf{$-$0.09} & \rd{rdO}{+0.9\,\textsuperscript{O}} & $-$0.01 & -- & $-$0.06 & -- & 0.00 & +2 \\
\addlinespace[2pt]
Impulses 0.05\% of samples & $-$0.01 & +9 & 0.00 & +0.7 & 0.00 & -- & $-$0.01 & -- & $-$0.02 & +0.5 & 0.00 & -- & +0.01 & -- & 0.00 & +1 \\
Impulses 0.5\% of samples & 0.00 & +4 & $-$0.08 & +3 & $-$0.01 & -- & $-$0.01 & -- & $-$0.09 & +1 & $-$0.01 & -- & \textbf{$-$0.31} & -- & +0.01 & +5 \\
Impulses 1\% of samples & $-$0.02 & +8 & \textbf{$-$0.17} & \rd{rdO}{+3\,\textsuperscript{O}} & $-$0.01 & -- & \textbf{$-$0.05} & -- & \textbf{$-$0.32} & \rd{rdO}{+2\,\textsuperscript{O}} & $-$0.01 & -- & \textbf{$-$0.36} & -- & +0.01 & +7 \\
\addlinespace[2pt]
Notch 50 Hz & 0.00 & +8 & 0.00 & 0 & 0.00 & -- & 0.00 & -- & 0.00 & +0.2 & 0.00 & -- & +0.04 & -- & 0.00 & +0.1 \\
\addlinespace[2pt]
60 Hz mains + 50 Hz notch & 0.00 & +0.8 & 0.00 & +0.1 & $-$0.01 & -- & $-$0.01 & -- & 0.00 & +0.2 & 0.00 & -- & +0.04 & -- & 0.00 & 0 \\
\addlinespace[2pt]
FGSM decrease, $\varepsilon$ = 0.01 & \textbf{$-$0.21} & \rd{rdU}{+4\,\textsuperscript{U}} & 0.00 & +0.2 & $-$0.02 & -- & \textbf{$-$0.05} & -- & +0.01 & $-$0.1 & 0.00 & -- & $-$0.01 & -- & +0.07 & $-$0.1 \\
FGSM decrease, $\varepsilon$ = 0.05 & \textbf{$-$0.56} & \rd{rdU}{+4\,\textsuperscript{U}} & \textbf{$-$0.53} & \rd{rdU}{$-$0.4\,\textsuperscript{U}} & \textbf{$-$0.09} & -- & \textbf{$-$0.20} & -- & \textbf{$-$0.47} & \rd{rdU}{+0.1\,\textsuperscript{U}} & $-$0.01 & -- & \textbf{$-$0.25} & -- & $-$0.05 & +0.3 \\
FGSM decrease, $\varepsilon$ = 0.10 & \textbf{$-$0.51} & \rd{rdU}{+2\,\textsuperscript{U}} & \textbf{$-$0.57} & \rd{rdU}{0\,\textsuperscript{U}} & \textbf{$-$0.14} & -- & \textbf{$-$0.43} & -- & \textbf{$-$0.47} & \rd{rdU}{0\,\textsuperscript{U}} & $-$0.01 & -- & \textbf{$-$0.38} & -- & \textbf{$-$0.09} & \rd{rdO}{+0.2\,\textsuperscript{O}} \\
\addlinespace[2pt]
FGSM increase, $\varepsilon$ = 0.01 & \textbf{$-$0.17} & \rd{rdO}{+6\,\textsuperscript{O}} & $-$0.03 & +0.1 & 0.00 & -- & $-$0.02 & -- & \textbf{$-$0.23} & \rd{rdU}{0\,\textsuperscript{U}} & $-$0.01 & -- & $-$0.12 & -- & \textbf{$-$0.04} & \rd{rdU}{0\,\textsuperscript{U}} \\
FGSM increase, $\varepsilon$ = 0.05 & \textbf{$-$0.29} & \rd{rdU}{+5\,\textsuperscript{U}} & \textbf{$-$0.23} & \rd{rdU}{+0.1\,\textsuperscript{U}} & +0.01 & -- & \textbf{$-$0.16} & -- & \textbf{$-$0.42} & \rd{rdU}{+0.1\,\textsuperscript{U}} & \textbf{$-$0.02} & -- & \textbf{$-$0.35} & -- & \textbf{$-$0.06} & \rd{rdO}{+0.2\,\textsuperscript{O}} \\
FGSM increase, $\varepsilon$ = 0.10 & \textbf{$-$0.29} & \rd{rdU}{+3\,\textsuperscript{U}} & \textbf{$-$0.26} & \rd{rdU}{0\,\textsuperscript{U}} & $-$0.01 & -- & \textbf{$-$0.27} & -- & \textbf{$-$0.45} & \rd{rdU}{$-$0.1\,\textsuperscript{U}} & \textbf{$-$0.02} & -- & \textbf{$-$0.39} & -- & \textbf{$-$0.06} & \rd{rdU}{+0.1\,\textsuperscript{U}} \\


==> tables/tab_summary.tex <==
SeizureTransformer & TUSZ & 0.62 & 5/17 & 1/13 & 6/6 & \makecell[l]{0.10\\{\scriptsize Impedance 0--1 Hz, 200 \textmu V}} & 0.07 & 14.5 \\
EEGNet & TUSZ & 0.57 & 5/17 & 4/13 & 4/6 & \makecell[l]{0.06\\{\scriptsize Impedance 0--1 Hz, 200 \textmu V}} & 0.01 & 9.6 \\
EEGWaveNet & TUSZ & 0.36 & 4/17 & 1/13 & 2/6 & \makecell[l]{0.26\\{\scriptsize Drift, 0.2 Hz sine, 50 \textmu V}} & 0.21 & 2.6 \\
EventNet & TUSZ & 0.71 & 5/17 & 6/13 & 5/6 & \makecell[l]{0.38\\{\scriptsize Impedance 0--1 Hz, 200 \textmu V}} & 0.28 & 12.2 \\
\addlinespace
EEGNet & Siena & 0.51 & 11/17 & 5/13 & 5/6 & \makecell[l]{0.14\\{\scriptsize Impedance 0--1 Hz, 200 \textmu V}} & 0.04 & 34.1 \\
EEGWaveNet & Siena & 0.08 & 0/17 & 1/13 & 2/6 & \makecell[l]{0.06\\{\scriptsize AWGN 0 dB SNR}} & 0.06 & 1.7 \\
EventNet & Siena & 0.46 & 1/17 & 5/13 & 4/6 & \makecell[l]{0.07\\{\scriptsize AWGN 0 dB SNR}} & 0.07 & 27.9 \\
\addlinespace
EEGNet & CHB-MIT & 0.09 & 3/17 & 0/13 & 4/6 & \makecell[l]{0.05\\{\scriptsize Band-pass 1--40 Hz}} & 0.00 & 3.8 \\

